MPL: Lifting 3D Human Pose from Multi-view 2D Poses

Estimating 3D human poses from 2D images is challenging due to occlusions and projective acquisition. Learning-based approaches have been largely studied to address this challenge, both in single and multi-view setups. These solutions however fail to generalize to real-world cases due to the lack of (multi-view) 'in-the-wild' images paired with 3D poses for training. For this reason, we propose combining 2D pose estimation, for which large and rich training datasets exist, and 2D-to-3D pose lifting, using a transformer-based network that can be trained from synthetic 2D-3D pose pairs. Our experiments demonstrate decreases up to 45% in MPJPE errors compared to the 3D pose obtained by triangulating the 2D poses. The framework's source code is available at https://github.com/aghasemzadeh/OpenMPL .

==> plots/compare_datasets.tex <==



\begin{figure}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tikzpicture}
        \begin{axis}[
            xbar,
            % width=\textwidth,
            % height=8cm,
            bar width=0.25cm,
            xlabel={Values},
            ylabel={Keypoints},
            symbolic y coords={lsho, rsho, lelb, relb, lwri, rwri, lkne, rkne, lank, rank, MPJPE},
            ytick=data,
            nodes near coords,
            legend style={at={(1.05,1)},anchor=north west},
            enlarge y limits=0.1,
            xticklabel style={/pgf/number format/fixed, /pgf/number format/precision=2},
        ]
        \addplot table [x=amass_gt, y=Keypoint, col sep=comma] {data.csv};
        \addplot table [x=amass_mmpose, y=Keypoint, col sep=comma] {data.csv};
        \addplot table [x=h36m_gt, y=Keypoint, col sep=comma] {data.csv};
        \addplot table [x=tri, y=Keypoint, col sep=comma] {data.csv};
        \legend{amass\_gt, amass\_mmpose, h36m\_gt, tri}
        \end{axis}
    \end{tikzpicture}
    }
    \caption{Comparison of Joint Positions and MPJPE}
    \label{fig:comparison}
\end{figure}


